Goal-Oriented Adaptivity and Multilevel Preconditioning for the Poisson-Boltzmann Equation

In this article, we develop goal-oriented error indicators to drive adaptive refinement algorithms for the Poisson-Boltzmann equation. Empirical results for the solvation free energy linear functional demonstrate that goal-oriented indicators are not sufficient on their own to lead to a superior refinement algorithm. To remedy this, we propose a problem-specific marking strategy using the solvation free energy computed from the solution of the linear regularized Poisson-Boltzmann equation. The convergence of the solvation free energy using this marking strategy, combined with goal-oriented refinement, compares favorably to adaptive methods using an energy-based error indicator. Due to the use of adaptive mesh refinement, it is critical to use multilevel preconditioning in order to maintain optimal computational complexity. We use variants of the classical multigrid method, which can be viewed as generalizations of the hierarchical basis multigrid and Bramble-Pasciak-Xu (BPX) preconditioners.

==> app.tex <==
%% rcsid="$Id: app.tex,v 1.1 2011-09-19 16:48:58 hrg Exp $"
%% --------------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\appendix
\section{Some key technical tools and some supporting results}
\label{sec:app}

\subsection{Algebraic formulation of multilevel preconditioning}
\mnote{SB: WARNING ... This material may be recycled from other papers}
In the uniform refinement setting, the parallelized or additive version of
the multigrid method, also known as the BPX preconditioner, is defined
as follows:
\begin{equation} \label{eqn:bpxImp}
X u := \sum_{j=0}^J 
2^{j(d-2)} \sum_{i=1}^{N_j} (u,\phi_i^{(j)}) \phi_i^{(j)},~~~u \in \calg{S}_J.
\end{equation}
Only in the presence of a geometric increase in the number of DOF,
the same assumption for optimality of a single classical
(i.e.~smoother acting on all DOF) multigrid or BPX iteration, does the cost 
per iteration remain optimal. In the case of local refinement, the BPX 
preconditioner (\ref{eqn:bpxImp}) (usually known as additive multigrid) 
can easily be suboptimal because of the suboptimal cost per iteration.  
If the smoother is restricted to the space generated by \emph{fine or newly 
created} basis functions,
i.e.~$\tilde{\calg{S}}_j := (I_j - I_{j-1})~\calg{S}_{j}$,
then~(\ref{eqn:bpxImp}) corresponds to the additive HB
preconditioner in~\cite{Yser86b}:
\begin{equation} \label{eqn:bpxHb}
X_{\mbox{{\tiny {\rm HB}}}} u =
\sum_{j=0}^J 2^{j(d-2)} \sum_{i=N_{j-1}+1}^{N_j} (u,\phi_i^{(j)}) \phi_i^{(j)},
~~~ u \in \calg{S}_J.
\end{equation}
However, the HB preconditioner suffers from a suboptimal iteration count.  
Namely, if the algebraic 
system~(\ref{algebraicSystem}) is preconditioned by the HB preconditioner, the 
arising condition number is $\calg{O}(J^2)$ and $\calg{O}(2^J)$ in 2D and 3D, respectively.

In the local refinement setting, in order to maintain optimal 
overall computational complexity, the remedy is to restrict the smoother 
to a local space $\tilde{\calg{S}}_j$ which is typically slightly larger 
than the one generated by basis functions corresponding to fine DOF:
\begin{equation} \label{subset:localSpace}
(I_j - I_{j-1})~\calg{S}_{j} \subseteq \tilde{\calg{S}}_j \subset \calg{S}_j,
\end{equation}
where $I_j:L_2(\Omega) \rightarrow \calg{S}_j$ denotes the finite
element interpolation operator. The subspace generated by the nodal
basis functions corresponding to \emph{fine or newly created} degrees
of freedom (DOF) on level $j$ is denoted by $(I_j - I_{j-1})~{\mathcal
S}_{j}$.  Nodes--equivalently, DOF--corresponding to $\tilde{{\mathcal
S}}_j$ and their cardinality will be denoted by $\tilde{\calg{N}}_j$
and $\tilde{N}_j$, respectively. The above deficiencies of the BPX and
HB preconditioners can be overcome by restricting the (smoothing)
operations to $\tilde{\calg{S}}_j$.  This leads us to define the BPX
preconditioner for the local refinement setting as:
\begin{equation} \label{id:BPX}
X u := \sum_{j=0}^J 2^{j(d-2)} \sum_{i \in \tilde{\calg{N}}_j}
(u,\phi_i^{(j)}) \phi_i^{(j)},~~~ u \in \calg{S}_J.
\end{equation}

\begin{remark}
In order to prove optimal results on convergence, the basic theoretical 
restriction on the refinement procedure is that the refinement regions
from each level forms a \emph{nested} sequence. 
Let $\Omega_j$ denote the refinement region, namely, the union of 
the supports of basis functions which are introduced at level $j$.
Due to nested refinement $\Omega_j \subset \Omega_{j-1}$. Then the 
following nested hierarchy holds:
$$
\Omega_J \subset \Omega_{J-1} \subset \cdots \subset \Omega_0 = \Omega.
$$
Simply, the restriction indicates that tetrahedra of level $j$ which
are not candidates for further refinement will never be touched in the
future.  In practice, depending on the situation, the above nestedness
restriction may or may not be enforced. We enforce the restriction in
Lemma~\ref{lemma:BEK}. In realistic situations, it is typically not
enforced.
\end{remark}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Matrix Representations and Local Smoothing}

We describe how to construct the matrix representation of the
preconditioners under consideration. Let the prolongation operator from
level $j-1$ to $j$ be denoted by
$$
P_{j-1}^j \in \Re^{\tilde{N}_j \times \tilde{N}_{j-1}},
$$
and also denote the prolongation operator from level $j$ to $J$ as:
$$
P_j \equiv P_j^J = P_{J-1}^J  \ldots P_j^{j+1} \in 
\Re^{N_J \times \tilde{N}_j},
$$
where $P_J^J$ is defined to be the rectangular identity matrix 
$I \in \Re^{N_J \times \tilde{N}_{J-1}}$. 
Then the matrix representation of (\ref{eqn:bpxImp}) becomes~\cite{XuQi94}:
$$
X = \sum_{j=0}^J 2^{j(d-2)} P_j P_j^t.
$$
One can also introduce a version with an explicit smoother $G_j$: 
$$
X = \sum_{j=0}^J P_j G_j P_j^t.
$$
Throughout this article, the smoother 
$G_j \in \Re^{\tilde{N}_j \times \tilde{N}_j}$ is a symmetric 
Gauss-Seidel  iteration. Namely, 
$G_j = (D_j + U_j)^{-1} D_j (D_j + L_j)^{-1}$ where
$A_j = D_j + L_j + U_j$ with $\tilde{N}_0 = N_0$.

The matrix representation of~(\ref{eqn:bpxHb}) is formed from matrices $H_j$
which are simply the tails of the $P_j$ corresponding to newly introduced DOF 
in the fine space. In other words, 
$H_j \in \Re^{N_J \times (N_j - N_{j-1})}$ is given by only keeping the fine 
columns (the last $N_j - N_{j-1}$ columns of $P_j$). Hence,
the matrix representation of~(\ref{eqn:bpxHb}) becomes:
$$
X_{\mbox{{\tiny {\rm HB}}}} = \sum_{j=0}^J 2^{j(d-2)} H_j H_j^t.
$$

If the sum over $i$ in (\ref{eqn:bpxImp}) is restricted only to those 
nodal basis functions with supports that intersect the refinement region
\cite{BoYs93,BrPa93,DaKu92,Oswa94}, then we obtain the set called as 
{\em one-ring} of fine DOF. Namely, the set which contains fine DOF and their
immediate neighboring coarse DOF: 
$${\rm ONERING}^{(j)}=\{onering (ii):~ii=N_{j-1}+1, \ldots, {N_j} \},$$
where $onering (ii) = \{ii, fathers(ii)\}.$
Now, the generic preconditioner~(\ref{id:BPX}) for local refinement 
transforms into the following preconditioner:
\begin{equation} \label{eqn:bpxLocal}
X u =
\sum_{j=0}^J 2^{j(d-2)}
\sum_{ i \in \mbox{{\tiny {\rm ONERING}}}^{(j)} }
(u,\phi_i^{(j)}) \phi_i^{(j)},
~~~ u \in \calg{S}_J.
\end{equation}

There are three popular choices for $\tilde{\calg{N}}_j$. 
We outline possible BPX choices by the following DOF corresponding to:
\begin{itemize}
\item {\bf (DOF-1)} The basis functions with supports that intersect 
the refinement region $\Omega_j$~\cite{BoYs93,BrPa93,DaKu92}. We call
this set $\mbox{{\tiny {\rm ONERING}}}^{(j)}$.
\item {\bf (DOF-2)} The basis functions with supports that are contained in 
$\Omega_j$~\cite{Oswa94}.
\item {\bf (DOF-3)} Created by red refinement and their corresponding coarse
DOF.
\end{itemize}
Here, red refinement refers to quadrasection or octasection in 2D and
3D, respectively.  Green refinement simply refers to bisection.

The interesting ones are DOF-1 and DOF-3 and we would like to
elaborate on these. In the numerical experiments reported
in~\cite{ABH02a}, DOF-1 was used. For the provably optimal
computational complexity result in Lemma~\ref{lemma:BEK} DOF-3 is
used.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Hierarchical Basis Methods, the Sets DOF-1, DOF-3, and Local Smoothing Computational Complexity}
\label{sec:onering}

HB methods exploit a 2-level hierarchical decomposition of the DOF. They
are divided into the coarse (the ones inherited from previous levels) and 
the fine (the ones that are newly introduced) nodes. In fact, in the operator
setting, this decomposition is a direct consequence of the direct decomposition
of the finite element space as follows:
$$\calg{S}_j = \calg{S}_{j-1} \oplus \calg{S}_j^f.$$
Hence, $A_j$ can be represented by a two-by-two block form:
\begin{equation}  \label{defn:2by2}
A_j =
\left[ \begin{array}{cc}
A_{j-1}    & A^{(j)}_{12} \\
A^{(j)}_{21} & A^{(j)}_{22}
\end{array} \right]
\begin{array}{ll}
\} & \calg{S}_{j-1} \\
\} & \calg{S}^f_j
\end{array},
\end{equation}
where $A_{j-1}$, $A^{(j)}_{12}$, $A^{(j)}_{21}$, and $A_{22}^{(j)}$
correspond to coarse-coarse, coarse-fine, fine-coarse, and fine-fine 
discretization operators respectively. The same 2-level decomposition 
carries directly to the matrix setting.

The set DOF-1 can be directly determined by the sparsity pattern of
the fine-fine subblock $A_{22}^{(j)}$ of the stiffness matrix
in~(\ref{defn:2by2}). Then, the set of DOF over which the BPX
preconditioner ~(\ref{eqn:bpxLocal}) smooths is simply the union of the
column locations of nonzero entries corresponding to fine DOF. Using
this observation, HB smoother can easily be modified to be a BPX
smoother.

DOF-3 is equivalent to the following set:
\begin{equation} \label{eqn:BEK-DOF}
\hspace*{-1.5cm}
\tilde{\calg{N}}_j = \{i=N_{j-1}+1, \ldots, N_j \}
\bigcup \{ i: \phi_i^{(j)} \neq \phi_i^{(j-1)},~~i=1, \ldots, N_{j-1}\},
\end{equation}
and the corresponding space over which the smoother acts:
$$
\tilde{\calg{S}}_j = {\rm span} \left[
\bigcup \{ \phi_i^{(j)} \}_{i=N_{j-1}+1}^{N_j}
\bigcup \{ \phi_i^{(j)} \neq \phi_i^{(j-1)} \}_{i=1}^{N_{j-1}} 
\right].
$$

This set is used in the Bornemann-Erdmann-Kornhuber (BEK)
refinement~\cite{BEK93} and we utilize this set for the estimates of
3D local refinement. Since green refinement simply bisects a simplex,
the modified basis function is the same as the one before the
bisection due to linear interpolation. So the set of DOF in
(\ref{eqn:BEK-DOF}) corresponds to DOF created by red refinement and
corresponding coarse DOF (father DOF). The following crucial result
from~\cite{BEK93} establishes a bound for the number of nodes used for
smoothing. This indicates that the BPX preconditioner has provably
optimal (linear) computational complexity per iteration on the
resulting 3D mesh produced by the BEK refinement procedure.

\begin{lemma} \label{lemma:BEK}
The total number of nodes used for smoothing satisfies the bound:
\begin{equation} \label{ineq:smoothBound}
\sum_{j=0}^J \tilde{N}_j \leq \frac{5}{3}N_J - \frac{2}{3}N_0.
\end{equation}
\end{lemma}
\begin{proof}
See~\cite[Lemma 1]{BEK93}.
\end{proof}


==> makefilex <==
#! make
##############################################################################
# Purpose: MCP (Mathematical and Computational Physics Group) paper makefile.
#
# Notes:   This makefile is used by the MCP group (Michael Holst's Research 
#          Group in the Mathematics and Physics Departments at UC San Diego)
#          to build latex papers using the fairly simple combination of 
#          pdflatex, amstex/amslatex, and pdf/png images.
#
# Targets: The makefile will auto-generate the following based on the
#          requested make target:
#
#            Main Targets:
#
#              pdfth   --> ${TARGET}.pdf via pdflatex
#              pdf     --> ${TARGET}.pdf via pdflatex + thumbpdf
#              dvi     --> ${TARGET}.dvi via latex
#              dvip    --> ${TARGET}.dvi|ps|pdf via latex + dvips + ps2pdf
#
#            Auxilliary Targets:
#
#              arx     --> zarxiv.tar.gz (gzipped tarball for arXiv)
#              clean   --> rm -f *.aux, *.dvi, etc
#              rclean  --> clean + rm *.ps *.bbl (careful!)
#              rrclean --> rclean + rm m.pdf mm.pdf ${TARGET}.pdf (careful!)
#
# Author:  Michael Holst
# Date:    Sat Dec 19 22:23:18 PST 2009
##############################################################################

default: pdf

TARGET=m

ARXIV_DIR=zarxiv
ARXIV_FILES=${TARGET}.tex ${TARGET}.bbl \
			environ.tex symbols.tex abs-arxiv.txt \
			abs.tex ack.tex app.tex conc.tex \
			sec1.tex sec2.tex sec3.tex sec4.tex sec5.tex sec6.tex \
			\
			onefas-iters-dof.png onefas-ratio-dof.png oscillations.png \
			refine4.pdf 1FAS_domain.pdf 1fas-energy-2nd-print.png \
			1fas-energy-split-print.png 1fas-global.pdf 1fas-goal-print.png \
			1fas-goal-split-print.png 1fas-split-dual.pdf \
			1fas-split-primal.pdf 1fas-unknowns.pdf

LATEX=latex
PDFLATEX=pdflatex
#PDFLATEX=pdflatex --shell-escape
BIBTEX=bibtex
#BIBTEX=./zbibtex

all : pdf arx

dvi :
	make clean
	${LATEX} ${TARGET}.tex
	-${BIBTEX} ${TARGET}
	${LATEX} ${TARGET}.tex
	${LATEX} ${TARGET}.tex
	-cp -f ${TARGET}.dvi mm.dvi

dvip : dvi
	dvips -N0 -P pdf -t letter -o ${TARGET}.ps mm.dvi
	ps2pdf ${TARGET}.ps
	-cp -f ${TARGET}.pdf mm.pdf

pdf :
	make clean
	${PDFLATEX} ${TARGET}
	-${BIBTEX} ${TARGET}
	${PDFLATEX} ${TARGET}
	${PDFLATEX} ${TARGET}
	-cp -f ${TARGET}.pdf mm.pdf

pdfth : pdf
	thumbpdf ${TARGET}
	${PDFLATEX} ${TARGET}
	rm -f thumb*.png
	-cp -f ${TARGET}.pdf mm.pdf

arx : ${TARGET}.bbl
	./makex ${ARXIV_DIR} ${ARXIV_FILES}

clean :
	rm -f *.aux *.dvi *.log *.lof *.lot *.toc *.blg *.idx *.out *.tpt

rclean :
	make clean
	rm -f *.ps *.bbl

rrclean :
	make rclean
	rm -f m.pdf mm.pdf ${TARGET}.pdf
	rm -rf ${ARXIV_DIR}


